Learning Multi-agent Action Coordination via Electing First-move Agent

Learning to coordinate actions among agents is essential in complicated multi-agent systems. Prior works are constrained mainly by the assumption that all agents act simultaneously, and asynchronous action coordination between agents is rarely considered. This paper introduces a bi-level multi-agent decision hierarchy for coordinated behavior planning. We propose a novel election mechanism in which we adopt a graph convolutional network to model the interaction among agents and elect a first-move agent for asynchronous guidance. We also propose a dynamically weighted mixing network to effectively reduce the misestimation of the value function during training. This work is the first to explicitly model the asynchronous multi-agent action coordination, and this explicitness enables to choose the optimal first-move agent. The results on Cooperative Navigation and Google Football demonstrate that the proposed algorithm can achieve superior performance in cooperative environments. Our code is available at \url{https://github.com/Amanda-1997/EFA-DWM}.

==> 1-intro.tex <==
\section{Introduction}
Multi-agent reinforcement learning (MARL) has made impressive achievements in complicated real-life applications, such as self-driving~\cite{cao2012self-driving}, traffic light control~\cite{kuyer2008traffic}, and StarCraft II~\cite{vinyals2019grandmaster}. 
As the natural properties of multi-agent systems, the complexity and uncertainty often require coordination among agents.
% \replaced{As the nature of multi-agent systems }{However}, the complexity and uncertainty \deleted{of multi-agent systems} often require \xdp{agent} coordination\deleted{ between agents}. 
A naive solution is to reduce the multi-agent problem to a single-agent one where a central controller is used to collaboratively model the joint actions. 
% \replaced{A}{The} naive solution \deleted{to promote coordination} is \replaced{to simplify}{reducing} the multi-agent problem to a single-agent one where \replaced{a}{the} central controller \replaced{is used to collaboratively}{can} model the joint actions\deleted{ collaboratively}. 
However, it requires exploring a joint action space that grows exponentially~\cite{bellman2015adaptive}. 
Thus,  decentralized policies are prioritized that allow agents to make decisions independently and simultaneously to effectively avoid the computational problem, but one of their challenges is the acquisition of coordinated behaviours.
% Thus, decentralized \replaced{policies are prioritized that allow}{policy allows} agents to make decisions independently and simultaneously to \xdp{effectively} avoid the \xdp{computational} problem \deleted{effectively}, but \replaced{one of their challenges is the acquisition of}{it is challenging to obtain} coordinated behaviours.
% \deleted{Therefore, it is imperative to study the coordinated policy that allows an individual agent to coordinate its action with another agent.} 
We provide an instance for intuitive understanding. 
There is only one single-plank bridge, and two persons cross the river from opposite directions. If they move  simultaneously, neither could succeed. 
The only solution is to cross one by one.
This example illustrates the importance of asynchronous decisions with a first-move agent, adequately eliminating the above dilemma.
Such an idea has been proven effective in game theory. In the Stackelberg leadership model~\cite{albaek1990stackelberg}, one firm moves first considering other firms' policies, and the others move sequentially taking the best response to the former firm.  
\xdp{These inspire us to consider optimal election of a first-move agent for asynchronous multi-agent action coordination.} \deleted{These further inspire us to explicitly model the asynchronous multi-agent action coordination via electing a first-move agent.}
% There is only one single-plank bridge\replaced{, and two persons cross the river from opposite directions.}{ for two people standing opposite to cross the river.} If \replaced{they move}{two people act} simultaneously, \replaced{neither could succeed}{none of them can cross the river}. The \xdp{only} solution is \replaced{to cross one by one}{that one crosses the river first, and the other cannot act until the first-move person passes}. 
% This example \replaced{illustrates the importance of asynchronous decisions with a first-move agent, adequately eliminating the above dilemma.}{indicates that a first-move agent for asynchronous decisions is important for promoting action coordination to adequately eliminate the similar dilemma.}
% This example indicates that the coordinated actions between agents can adequately eliminate the dilemma. 
% Such an idea has \deleted{also} been proven effective in game theory\replaced{. In}{, where} the Stackelberg leadership model~\cite{albaek1990stackelberg}\replaced{,}{  is a strategic game in which} one firm moves first considering other firms' policies\replaced{, and}{. Then} the others move sequentially taking the best response to the former firm\replaced{.}{, repeating until the optimal equilibrium.} 
  

Several works recognize the importance of action coordination. BiAC~\cite{zhang2020bilevel} addresses the bi-level decision in MARL but mainly focuses on two agents. The multi-agent rollout algorithm~\cite{bertsekas2019multiagent_rollout} provides a theoretical view of asynchronous action execution. 
% \deleted{us with} a theoretical view of \replaced{asynchronous action execution}{ executing an asynchronous action rollout}.
DCG~\cite{bohmer2020dcg}, DICG~\cite{li2021dicg}, and DGN~\cite{jiang2018dgn} use coordination graphs to pass messages before the decision making process, but all agents take actions simultaneously, which would be stuck with the dilemma for some coordination tasks.
% These works 
\replaced{These works}{Although these works investigate action coordination, they} do not yet provide an explicit solution to obtain coordinated behaviors among multiple agents\deleted{ from the perspective of game theory}.\xdp{why explicit?}

In this paper, we propose a new \xdp{hierarchical} framework \replaced{of coordinated behaviour learning in MARL}{for MARL to learn coordinated behaviours inspired by the Stackelberg leadership model}. We aim to promote asynchronous action coordination via Electing the First-move Agent followed by a Dynamically Weighted Mixing network (\nameone) in cooperative multi-agent reinforcement learning. In the EFA module, we use the graph convolutional network (GCN)~\cite{kipf2016gcn} to aggregate the message from neighbours for a richer feature embedding, which is then used to elect the first-move agent.
In the DWM module, we use the weighted mixing network to place more emphasis on better joint action to the overall system dynamically.

The contributions of our work are three-fold.
\begin{itemize}
    \item We introduce a novel framework to construct a bi-level decision hierarchy to promote asynchronous action coordination for multiple agents.
    \item We propose to use a GCN-based election mechanism to select the optimal first-move agent and adopt the dynamically weighted mixing network to alleviate the problem of misestimation for value function.
    \item Empirical evaluations on several challenging MARL benchmarks \replaced{demonstrate the significant performance of the proposed method.}{show that our method can significantly achieve better performance.}
\end{itemize}




% \textbf{Contributions.} In this paper, we give a novel problem formulation based on partially observable Markov games which can enable coordination due to the asymmetry of the agents. 
% Under this formulation, we propose an algorithm called~\nameone~that aims at promoting coordination through Electing the First-move Agent followed by an improved Deep Q-Network in cooperative multi-agent reinforcement learning. 
% % Furthermore, we provide a convergence analysis of the approach~\nameone. 
% In the EFA sub-module, we construct a coordinated graph and use the graph convolutional network to aggregate the message from neighbours for a richer feature embedding used to elect the first-move agent. In the DQN sub-module, we use the weighted mixing network to places more emphasis on better joint action and impose a counterfactual constraint for the first-move agent to encourage more contribution of the first-move agent to the overall system.
% The empirical evaluations on several challenging MARL benchmarks show that our method can significantly achieve better performance and faster convergence over other related methods. These results provide a new
% perspective in understanding and promoting the emergence of coordination among agents and demonstrate that our algorithm has broad prospects for addressing many complex real-world problems.



% Recently we have witnessed the impressive achievement of deep reinforcement learning (DRL) for Atari~\cite{mnih2013playingatari},  OpenAI Gym~\cite{Brockman2016openaigym} and Go~\cite{silver2017mastering, schrittwieser2020mastering}. The more complicated example, such as self-driving~\cite{cao2012self-driving}, traffic light control~\cite{kuyer2008traffic} and StarCraft II~\cite{vinyals2019grandmaster} can be modeled as multi-agent systems (MAS)~\cite{shoham2008mas}. 
% The complexity and uncertainty of multi-agent systems make it imperative to study the coordination among the agents. 
% % However, in these complex applications, learning coordination is abstract and difficult.
% For instance, there is only one single-plank bridge for two people standing opposite to cross the river. If two people act simultaneously, none of them can cross the river. The solution is one crosses the river first, and the other cannot act until the first-move person passes.
% Borrowing from the human society for the multi-agent system is essential for better collaboration and feasible solutions. However, learning coordination is abstract and how to design a mechanism to promote the coordination is extremely difficult. 

% The past few decades have seen increasingly rapid advances in the field of collaborative multi-agent reinforcement learning (MARL), where the agents learn to coordinate to achieve joint success. There is a growing body of literature that recognizes the importance of coordination.
% %, exemplified in ~\cite{lowe2017maddpg, iqbal2019actor, wang2020dop, yang2020Q-DPP, hu2021updet, ZhangSTGMB2020Robust}.  
% Among them, learning communication protocol~\cite{foerster2016RIAL&DIAL, sukhbaatar2016CommNet, jiang2018atoc, das2019tarmac} has been proposed to learn the coordinated behaviour among multiple agents. 
% Some works~\cite{ahilan2019feudal, tessler2017deephrl} are goal-oriented, which employ a hierarchy with managers and workers to enforce the workers to achieve the goal generated by managers.
% There are also some works~\cite{wang2020rode, wang2020roma} that assign the agents with different roles in order to achieve better coordination to reach the final success.
% However, in these settings formulated by Markov Games~\cite{littman1994markov}, all agents are regarded symmetrically and take actions simultaneously, which would be stuck with the dilemma for some coordination tasks. Much of the research up to now has not fundamentally solved the coordination problem in multi-agent reinforcement learning. 

% In order to eliminate the coordination dilemma, we introduce a new framework for MARL to learn coordinated behaviour. The core idea is that we elect a first-move agent among all the agents to act first, and other agents take their best response to the first-move agent. 
% We break the symmetry and endow the hierarchical order of play for the agents to obtain better coordination. 
% We develop our system in the context of cooperative multi-agent reinforcement learning, where there is a single goal to be optimized by maximizing a shared global cumulative return.


% This work will generate fresh insight into 

% regularizing the expected cumulative reward with mutual information
% among agents’ actions induced by injecting a latent variable.


% has broad prospects for addressing many complex real-world problems




% \textbf{Contributions.} In this paper, we give a novel problem formulation based on partially observable Markov games which can enable coordination due to the asymmetry of the agents. 
% Under this formulation, we propose an algorithm called~\nameone~that aims at promoting coordination through Electing the First-move Agent followed by an improved Deep Q-Network in cooperative multi-agent reinforcement learning. 
% % Furthermore, we provide a convergence analysis of the approach~\nameone. 
% In the EFA sub-module, we construct a coordinated graph and use the graph convolutional network to aggregate the message from neighbours for a richer feature embedding used to elect the first-move agent. In the DQN sub-module, we use the weighted mixing network to places more emphasis on better joint action and impose a counterfactual constraint for the first-move agent to encourage more contribution of the first-move agent to the overall system.
% The empirical evaluations on several challenging MARL benchmarks show that our method can significantly achieve better performance and faster convergence over other related methods. These results provide a new
% perspective in understanding and promoting the emergence of coordination among agents and demonstrate that our algorithm has broad prospects for addressing many complex real-world problems.
% effectiveness 

% This paper is organized as follows. 
% This paper has been organised in the following way.
% The remaining part of the paper proceeds as follows:
% Firstly, we discuss the relevant literature in Section 2.
% Then we introduce the partially observable Markov game, graph convolutional network and value-based multi-agent reinforcement learning in Section 3.
% Next, Section 4 is concerned with the methodology used for this paper. We explain the problem formulation and present the detailed framework description. 
% Afterwards, we explore our algorithm in several complex tasks and make an analysis. 
% Finally, the conclusion is provided in Section 6.


















==> 2-Related_work.tex <==
\section{Related Work}
% We now discuss the body of the relevant literature. 

% Recently, the \textit{centralized training with decentralized execution}(CTDE) paradigm has attracted more and more attention from researchers due to its capacity of alleviating the non-stationarity brought by the decentralized approach and the poor scalability of the centralized approach. 
% MADDPG~\cite{lowe2017maddpg} and MAAC~\cite{iqbal2019actor} are the multi-agent extension of deterministic policy gradient algorithms~\cite{lillicrap2016ddpg, silver2014deterministic}, learns the centralized critic to train a decentralized policy for each agent. 
% COMA~\cite{foerster2018COMA} updates stochastic policies using the counterfactual gradients and deals with the issue of credit assignment.
% PS-TRPO~\cite{gupta2017pstrpo} uses a decentralized policy network with an appropriate training protocol for better scalability.
% More recent studies, such as \cite{wang2020dop, yang2020Q-DPP, hu2021updet, ZhangSTGMB2020Robust}, take advantage of CTDE to provide solutions for training
% agents in complex multi-agent environments and achieve better coordination. 
% Similar to the CTDE setting, our method also enjoys decentralized execution with the centralized critic.

% empowering the agent to learn cooperative behavior considering other agents’policies without any communication in distributed execution.

 
%CTDE has an important concept, Individual-Global-Max (IGM) principle, which requires the consistency between joint and local action selections to support efficient local decision-making. However, in order to achieve scalability, existing MARL methods either limit representation expressiveness of their value function classes or relax the IGM consistency, which may suffer from instability risk or may not perform well in complex domains.

% Qmix-based
Recently, the \textit{centralized training with decentralized execution}(CTDE) paradigm has attracted more and more attention from researchers due to its capacity of alleviating the non-stationarity brought by the decentralized approach and the poor scalability of the centralized approach. 
Combining the CTDE regime with value-based solutions, some works show great superiority in multi-agent reinforcement learning (MARL) tasks. The structural constraints in factorization such as the additivity of VDN~\cite{sunehag2018vdn}, FQL~\cite{zhou2019fql} and the monotonicity of QMIX~\cite{rashid2018qmix}, WQMIX~\cite{RashidFPW2020wqmix} naturally limit the scope of their applications. QTRAN~\cite{son2019qtran}, which is free from such structural constraints, guarantees more general factorization than VDN or QMIX. However, relaxing the optimization constraints by two penalties deviates QTRAN from exact solutions. 
%QTRAN++~\cite{} resolves the limitations of QTRAN by stabilizing the training objective and introducing a multi-head mixing network.
Qatten~\cite{yang2020Qatten} introduce multi-head attention to establish the mixing network. MAVEN~\cite{MahajanRSW19MAVEN} hybridizes value and policy-based methods by introducing a latent space for hierarchical control. 
QPLEX~\cite{wang2021qplex} takes a duplex duelling network architecture to factorize the joint value function and enables efficient value function learning.
In this paper, we also utilize the value-decomposition popularized recently to address the complex multi-agent problems, which belongs to the Q-learning family.

Role-based works are broadly related to our method, but the difference is that we only elect the first-move agent. 
In some works~\cite{lhaksmana2018role, ryu2020hama, wu2020AGONet}, roles are predefined using prior knowledge, which hurts generalization of the policy and requires prior knowledge that may not be available in practice. To alleviate this issue, the Bayesian Policy Search approach for MARL~\cite{wilson2010bayesian} is proposed to demonstrate the practical discovery of roles from supervised trajectories, and ROMA~\cite{wang2020roma} learns a role encoder to generate the role embedding for the emergence of roles. RODE~\cite{wang2020rode} learns a role selector based on action effects to make the role discovery much more accessible. 
However,  our work aims to elect a role, i.e. the first-move agent, not to divide all agents into roles for better coordination. 



Learning coordinated behaviour in multi-agent systems are studied extensively in the MARL community. Some previous works attempt to promote coordination by communication which can enhance the collective intelligence of learning agents further. RIAL, DIAL~\cite{foerster2016RIAL&DIAL}, CommNet~\cite{sukhbaatar2016CommNet}, BiCNet~\cite{peng2017bicnet}, Message-Dropout~\cite{kim2019message-dropout}, ATOC~\cite{jiang2018atoc}, MAGIC~\cite{niu2021magic} and SchedNet~\cite{kim2018scheNet} attempt to learn an efficient communication protocol in the decentralized execution phase for various multi-agent tasks. 
Some impressive work like ~\cite{mordatch2018emergence, lazaridou2020language, lazaridou2020emergent, havrylov2017emergence} try to figure out the possibility of the artificial emergence of language for communication.
However, unlike the above work, we do not communicate explicitly but promote coordination through the information transmission from the first-move agent to other agents.


